Massive particles and unitarity cuts

We present an extension of the spinor integration formalism of one loop amplitudes from the double-cut to the single-cut case. This technique can be applied for the computation of the tadpole coefficients. Moreover we describe an off-shell continuation of one loop amplitudes that allows a finite evaluation of the unitarity cuts in the channel of a single massive external fermion.

==> DIAGRAMS/HBBct.tex <==
\unitlength=0.42bp%
\scriptsize 
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{$H(k_1)$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{$b(k_2,c_2)$}
\FAProp(20.,5.)(15.5,7.5)(0.,){/Straight}{1}
\FALabel(17.4773,5.37506)[tr]{$b(k_3,c_3)$}
\FAProp(15.5,7.5)(11.,10.)(0.,){/Straight}{1}
\FALabel(12.9773,7.87506)[tr]{$b$}
\FAVert(11.,10.){0}
\FAVert(15.5,7.5){2}
\end{feynartspicture}
%
% 
\hspace{0.3cm}
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{$H(k_1)$}
\FAProp(20.,15.)(15.5,12.5)(0.,){/Straight}{-1}
\FALabel(17.4773,14.6249)[br]{$b(k_2,c_2)$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{$b(k_3,c_3)$}
\FAProp(15.5,12.5)(11.,10.)(0.,){/Straight}{-1}
\FALabel(12.9773,12.1249)[br]{$b$}
\FAVert(11.,10.){0}
\FAVert(15.5,12.5){2}
\end{feynartspicture}
%
%


==> DIAGRAMS/HBBloop.tex <==
\unitlength=0.42bp%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(6.5,10.)(0.,){/ScalarDash}{0}
\FALabel(3.25,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(13.,14.)(0.,){/Straight}{-1}
\FALabel(16.2808,15.5544)[b]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(13.,6.)(0.,){/Straight}{1}
\FALabel(16.2808,4.44558)[t]{\scriptsize $b(k_3,c_3)$}
\FAProp(6.5,10.)(13.,14.)(0.,){/Straight}{1}
\FALabel(9.20801,13.1807)[br]{\scriptsize $b$}
\FAProp(6.5,10.)(13.,6.)(0.,){/Straight}{-1}
\FALabel(9.20801,6.81927)[tr]{\scriptsize $b$}
\FAProp(13.,14.)(13.,6.)(0.,){/Cycles}{0}
\FALabel(14.974,10.)[l]{\scriptsize $g$}
\FAVert(6.5,10.){0}
\FAVert(13.,14.){0}
\FAVert(13.,6.){0}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(17.3,6.5)(0.,){/Straight}{1}
\FALabel(18.9227,6.62494)[bl]{\scriptsize $b(k_3,c_3)$}
\FAProp(11.,10.)(13.7,8.5)(0.,){/Straight}{-1}
\FALabel(12.0773,8.37506)[tr]{\scriptsize $b$}
\FAProp(17.3,6.5)(13.7,8.5)(-0.8,){/Straight}{1}
\FALabel(14.4273,5.18506)[tr]{\scriptsize $b$}
\FAProp(17.3,6.5)(13.7,8.5)(0.8,){/Cycles}{0}
\FALabel(16.5727,9.81494)[bl]{\scriptsize $g$}
\FAVert(11.,10.){0}
\FAVert(17.3,6.5){0}
\FAVert(13.7,8.5){0}
%\FALabel(10.,-1.)[b]{$\mathcal{M}_{H\to b \bar b}(k_1,k_2,k_3)$}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(17.3,13.5)(0.,){/Straight}{-1}
\FALabel(18.3773,15.1249)[br]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(11.,10.)(13.7,11.5)(0.,){/Straight}{1}
\FALabel(12.0773,11.6249)[br]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(-0.8,){/Straight}{-1}
\FALabel(16.5727,10.1851)[tl]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(0.8,){/Cycles}{0}
\FALabel(13.4273,13.8149)[br]{\scriptsize $g$}
\FAVert(11.,10.){0}
\FAVert(17.3,13.5){0}
\FAVert(13.7,11.5){0}
\end{feynartspicture}



==> DIAGRAMS/HBBloopMOMon.tex <==
\unitlength=0.35bp%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(6.5,10.)(0.,){/ScalarDash}{0}
\FALabel(3.25,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(13.,14.)(0.,){/Straight}{-1}
\FALabel(16.2808,15.5544)[b]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(13.,6.)(0.,){/Straight}{1}
\FALabel(16.2808,4.44558)[t]{\scriptsize $b(k_3,c_3)$}
\FAProp(6.5,10.)(13.,14.)(0.,){/Straight}{1}
%\FALabel(9.20801,13.1807)[br]{\scriptsize $b$}
\FAProp(6.5,10.)(13.,6.)(0.,){/Straight}{-1}
%\FALabel(9.20801,6.81927)[tr]{\scriptsize $b$}
\FAProp(13.,14.)(13.,6.)(0.,){/Cycles}{0}
%\FALabel(14.974,10.)[l]{\scriptsize $g$}
\FAVert(6.5,10.){0}
\FAVert(13.,14.){0}
\FAVert(13.,6.){0}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{\scriptsize $b(k_2,c_2)$}
\FAProp(20.,5.)(17.3,6.5)(0.,){/Straight}{1}
%\FALabel(18.9227,6.62494)[bl]{\scriptsize $b$}
\FAProp(11.,10.)(13.7,8.5)(0.,){/Straight}{-1}
%\FALabel(12.0773,8.37506)[tr]{\scriptsize $b$}
\FAProp(17.3,6.5)(13.7,8.5)(-0.8,){/Straight}{1}
\FALabel(14.4273,5.18506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(17.3,6.5)(13.7,8.5)(0.8,){/Cycles}{0}
%\FALabel(16.5727,9.81494)[bl]{\scriptsize $g$}
\FAVert(11.,10.){0}
\FAVert(17.3,6.5){0}
\FAVert(13.7,8.5){0}
\FALabel(10.,-1.)[b]{$\mathcal{M}_{H\to b \bar b}(k_1,k_2,k_3)$}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{\scriptsize $H(k_1)$}
\FAProp(20.,15.)(17.3,13.5)(0.,){/Straight}{-1}
%\FALabel(18.3773,15.1249)[br]{\scriptsize $b$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(11.,10.)(13.7,11.5)(0.,){/Straight}{1}
%\FALabel(12.0773,11.6249)[br]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(-0.8,){/Straight}{-1}
%\FALabel(16.5727,10.1851)[tl]{\scriptsize $b$}
\FAProp(17.3,13.5)(13.7,11.5)(0.8,){/Cycles}{0}
\FALabel(14.4273,14.8149)[br]{\scriptsize $b(k_2,c_2)$}
\FAVert(11.,10.){0}
\FAVert(17.3,13.5){0}
\FAVert(13.7,11.5){0}
\end{feynartspicture}



==> DIAGRAMS/HBBtree.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,10.)(11.,10.)(0.,){/ScalarDash}{0}
\FALabel(5.5,9.18)[t]{$H$}
\FAProp(20.,15.)(11.,10.)(0.,){/Straight}{-1}
\FALabel(15.2273,13.3749)[br]{$b$}
\FAProp(20.,5.)(11.,10.)(0.,){/Straight}{1}
\FALabel(15.2273,6.62506)[tr]{$b$}
\FAVert(11.,10.){0}
\end{feynartspicture}



==> DIAGRAMS/HBBtreeC.tex <==
\unitlength=0.42bp%
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
\FAProp(18.,16.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
\FAProp(18.,4.)(9.,10.)(0.,){/Straight}{1}
\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
\FAProp(9.3,9.8)(18.,9.8)(0.,){/Cycles}{0}
\FALabel(15.,8.4)[dl]{\scriptsize $g(k_4,A_4)$}
\FAVert(9.,10.){-1}
\FALabel(9.,10.)[]{\scriptsize $T$}
\FALabel(10.,0.)[b]{$\mathcal{M}_{H\to b g \bar b}(k_1,k_2,k_4,k_3)$}
\end{feynartspicture}
%
%
\hspace{0.1cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(9.,10.)(0.,){/Cycles}{0}
\FALabel(4.22725,11.6251)[tr]{\scriptsize $g (k_1,A_1)$}
\FAProp(0.,5.)(9.,10.)(0.,){/Straight}{1}
\FALabel(4.77275,6.62506)[tl]{\scriptsize $b (k_2, c_2)$}
\FAProp(20.,10.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(14.5,11.07)[b]{\scriptsize $b (k_3, c_3)$}
\FAVert(9.,10.){0}
\FALabel(10.,0.)[b]{$\mathcal{M}_{g b \to b}(k_1,k_2,k_3)$}
\end{feynartspicture}
%
%
\hspace{0.1cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(9.,10.)(0.,){/Cycles}{0}
\FALabel(4.22725,11.6251)[tr]{\scriptsize $g (k_1,A_1)$}
\FAProp(0.,5.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(4.77275,6.62506)[tl]{\scriptsize $b (k_2, c_2)$}
\FAProp(20.,10.)(9.,10.)(0.,){/Straight}{+1}
\FALabel(14.5,11.07)[b]{\scriptsize $b (k_3, c_3)$}
\FAVert(9.,10.){0}
\FALabel(10.,0.)[b]{$\mathcal{M}_{g \bar b \to \bar b}(k_1,k_2,k_3)$}
\end{feynartspicture}


==> DIAGRAMS/HBBtreeS.tex <==
\unitlength=0.35bp%
%
%
\hspace{3cm}
% 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(9.,10.)(0.,){/ScalarDash}{0}
\FAProp(0.,6.)(9.,10.)(0.,){/Straight}{1}
\FALabel(0.,12.8)[t]{\scriptsize $H (k_1)$}
\FALabel(0.,7.2)[tr]{\scriptsize $b (k_2,c)$}
\FAProp(18.,16.)(9.,10.)(0.,){/Straight}{-1}
\FALabel(14,14)[br]{\scriptsize $b (k_3, c_3)$}
\FAProp(18.,4.)(9.,10.)(0.,){/Straight}{1}
\FALabel(14.,6.)[tr]{\scriptsize $b(k_5,c_5)$}
\FAProp(9.,10.)(18.,10.)(0.,){/Straight}{1}
\FALabel(15.,8.5)[dl]{\scriptsize $b(k_4,c)$}
\FAVert(9.,10.){-1}
\FALabel(9.,10.)[]{\scriptsize $T$}
\FALabel(10.,-1.)[b]{$\mathcal{M}_{H b\to b b \bar b}(k_1,\ell,k_3,\ell,k_5)$}
\end{feynartspicture}
%
%
\hspace{3cm}
% 
%


==> DIAGRAMS/QQTTloop.tex <==
%\unitlength=0.2bp% THIS IF U WANT TWO LINES OF SIX
\unitlength=0.25bp% THIS IF U WANT THREE LINES OF FOUR
\scriptsize
%
% 1
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$q$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$q$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Straight}{-1}
\FALabel(17.4558,15.2213)[b]{$t$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Straight}{1}
\FALabel(17.4558,4.77869)[t]{$t$}
\FAProp(4.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(7.,11.77)[b]{$g$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Cycles}{0}
\FALabel(17.77,10.)[l]{$g$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Straight}{-1}
\FALabel(12.699,12.6089)[br]{$t$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Straight}{1}
\FALabel(12.699,7.39114)[tr]{$t$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}
\end{feynartspicture}
%
% 2
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$q$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$q$}
\FAProp(20.,15.)(16.,13.5)(0.,){/Straight}{-1}
\FALabel(17.4558,15.2213)[b]{$t$}
\FAProp(20.,5.)(16.,6.5)(0.,){/Straight}{1}
\FALabel(17.4558,4.77869)[t]{$t$}
\FAProp(4.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(7.,11.77)[b]{$g$}
\FAProp(16.,13.5)(16.,6.5)(0.,){/Straight}{-1}
\FALabel(17.07,10.)[l]{$t$}
\FAProp(16.,13.5)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.699,12.6089)[br]{$g$}
\FAProp(16.,6.5)(10.,10.)(0.,){/Cycles}{0}
\FALabel(12.3463,6.7865)[tr]{$g$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}
\end{feynartspicture}
%
% 3
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){/Straight}{1}
\FALabel(2.54424,15.2213)[b]{$q$}
\FAProp(0.,5.)(4.,6.5)(0.,){/Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$q$}
\FAProp(20.,15.)(16.,10.)(0.,){/Straight}{-1}
\FALabel(17.2697,12.9883)[br]{$t$}
\FAProp(20.,5.)(16.,10.)(0.,){/Straight}{1}
\FALabel(18.7303,7.98828)[bl]{$t$}
\FAProp(16.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(13.,8.23)[t]{$g$}
\FAProp(4.,13.5)(4.,6.5)(0.,){/Cycles}{0}
\FALabel(2.93,10.)[r]{$g$}
\FAProp(4.,13.5)(10.,10.)(0.,){/Straight}{1}
\FALabel(7.301,12.6089)[bl]{$q$}
\FAProp(4.,6.5)(10.,10.)(0.,){/Straight}{-1}
\FALabel(7.301,7.39114)[tl]{$q$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}
\end{feynartspicture}
%
% 4
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){/Straight}{1}
\FALabel(2.54424,15.2213)[b]{$q$}
\FAProp(0.,5.)(4.,6.5)(0.,){/Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$q$}
\FAProp(20.,15.)(16.,10.)(0.,){/Straight}{-1}
\FALabel(17.2697,12.9883)[br]{$t$}
\FAProp(20.,5.)(16.,10.)(0.,){/Straight}{1}
\FALabel(18.7303,7.98828)[bl]{$t$}
\FAProp(16.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(13.,8.23)[t]{$g$}
\FAProp(4.,13.5)(4.,6.5)(0.,){/Straight}{1}
\FALabel(2.93,10.)[r]{$q$}
\FAProp(4.,13.5)(10.,10.)(0.,){/Cycles}{0}
\FALabel(7.65371,13.2135)[bl]{$g$}
\FAProp(4.,6.5)(10.,10.)(0.,){/Cycles}{0}
\FALabel(7.301,7.39114)[tl]{$g$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}
\end{feynartspicture}
\begin{feynartspicture}(300,300)(1,1)
%
% 5
%
\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$q$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$q$}
\FAProp(20.,15.)(13.5,13.5)(0.,){/Straight}{-1}
\FALabel(16.4015,15.2803)[b]{$t$}
\FAProp(20.,5.)(13.5,6.5)(0.,){/Straight}{1}
\FALabel(16.4015,4.71969)[t]{$t$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FALabel(5.43,10.)[r]{$q$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Cycles}{0}
\FALabel(10.,15.27)[b]{$g$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FALabel(10.,5.43)[t]{$g$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){/Straight}{-1}
\FALabel(14.57,10.)[l]{$t$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\end{feynartspicture}
%
% 6
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){/Straight}{1}
\FALabel(3.59853,15.2803)[b]{$q$}
\FAProp(0.,5.)(6.5,6.5)(0.,){/Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$q$}
\FAProp(20.,15.)(13.5,6.5)(0.,){/Straight}{-1}
\FALabel(17.9814,13.8219)[br]{$t$}
\FAProp(20.,5.)(13.5,13.5)(0.,){/Straight}{1}
\FALabel(17.8314,6.42814)[tr]{$t$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){/Straight}{1}
\FALabel(5.43,10.)[r]{$q$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){/Cycles}{0}
\FALabel(10.,15.27)[b]{$g$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){/Cycles}{0}
\FALabel(10.,5.43)[t]{$g$}
\FAProp(13.5,6.5)(13.5,13.5)(0.,){/Straight}{-1}
\FALabel(12.43,10.)[r]{$t$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,6.5){0}
\FAVert(13.5,13.5){0}
\end{feynartspicture}
%
% 7
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){/Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$q$}
\FAProp(0.,5.)(4.,10.)(0.,){/Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$q$}
\FAProp(20.,15.)(16.,10.)(0.,){/Straight}{-1}
\FALabel(17.2697,12.9883)[br]{$t$}
\FAProp(20.,5.)(16.,10.)(0.,){/Straight}{1}
\FALabel(18.7303,7.98828)[bl]{$t$}
\FAProp(4.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(7.,8.93)[t]{$g$}
\FAProp(16.,10.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(13.,8.23)[t]{$g$}
\FAProp(10.,10.)(10.,10.)(10.,15.){/Cycles}{0}
\FALabel(10.,16.07)[b]{$g$}
\FAVert(4.,10.){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}
\end{feynartspicture}
%
%  8
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$q$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$q$}
\FAProp(20.,15.)(17.,10.)(0.,){/Straight}{-1}
\FALabel(17.6509,12.8175)[br]{$t$}
\FAProp(20.,5.)(17.,10.)(0.,){/Straight}{1}
\FALabel(19.3491,7.81747)[bl]{$t$}
\FAProp(3.,10.)(7.,10.)(0.,){/Cycles}{0}
\FALabel(5.,11.77)[b]{$g$}
\FAProp(17.,10.)(13.,10.)(0.,){/Cycles}{0}
\FALabel(15.,8.23)[t]{$g$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Straight}{-1}
\FALabel(10.,6.53)[t]{$q'$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Straight}{1}
\FALabel(10.,13.47)[b]{$q'$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}
\end{feynartspicture}
%
% 9
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$q$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$q$}
\FAProp(20.,15.)(17.,10.)(0.,){/Straight}{-1}
\FALabel(17.6509,12.8175)[br]{$t$}
\FAProp(20.,5.)(17.,10.)(0.,){/Straight}{1}
\FALabel(19.3491,7.81747)[bl]{$t$}
\FAProp(3.,10.)(7.,10.)(0.,){/Cycles}{0}
\FALabel(5.,11.77)[b]{$g$}
\FAProp(17.,10.)(13.,10.)(0.,){/Cycles}{0}
\FALabel(15.,8.23)[t]{$g$}
\FAProp(7.,10.)(13.,10.)(0.8,){/GhostDash}{-1}
\FALabel(10.,6.53)[t]{$\eta$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/GhostDash}{1}
\FALabel(10.,13.47)[b]{$\eta$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}
\end{feynartspicture}
%
%  10
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){/Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$q$}
\FAProp(0.,5.)(3.,10.)(0.,){/Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$q$}
\FAProp(20.,15.)(17.,10.)(0.,){/Straight}{-1}
\FALabel(17.6509,12.8175)[br]{$t$}
\FAProp(20.,5.)(17.,10.)(0.,){/Straight}{1}
\FALabel(19.3491,7.81747)[bl]{$t$}
\FAProp(3.,10.)(7.,10.)(0.,){/Cycles}{0}
\FALabel(5.,11.77)[b]{$g$}
\FAProp(17.,10.)(13.,10.)(0.,){/Cycles}{0}
\FALabel(15.,8.23)[t]{$g$}
\FAProp(7.,10.)(13.,10.)(0.8,){/Cycles}{0}
\FALabel(10.,6.53)[t]{$g$}
\FAProp(7.,10.)(13.,10.)(-0.8,){/Cycles}{0}
\FALabel(10.,13.47)[b]{$g$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}
\end{feynartspicture}
%
%  11
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$q$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$q$}
\FAProp(20.,15.)(14.,10.)(0.,){/Straight}{-1}
\FALabel(16.4877,13.2107)[br]{$t$}
\FAProp(20.,5.)(18.2,6.5)(0.,){/Straight}{1}
\FALabel(19.6123,6.46074)[bl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(10.,8.93)[t]{$g$}
\FAProp(14.,10.)(15.8,8.5)(0.,){/Straight}{-1}
\FALabel(15.4123,9.96074)[bl]{$t$}
\FAProp(18.2,6.5)(15.8,8.5)(-0.8,){/Straight}{1}
\FALabel(15.6877,5.82926)[tr]{$t$}
\FAProp(18.2,6.5)(15.8,8.5)(0.8,){/Cycles}{0}
\FALabel(18.3123,9.17074)[bl]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(18.2,6.5){0}
\FAVert(15.8,8.5){0}
\end{feynartspicture}
%
% 12
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$q$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$q$}
\FAProp(20.,15.)(18.2,13.5)(0.,){/Straight}{-1}
\FALabel(18.5877,14.9607)[br]{$t$}
\FAProp(20.,5.)(14.,10.)(0.,){/Straight}{1}
\FALabel(17.5123,8.21074)[bl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(10.,8.93)[t]{$g$}
\FAProp(14.,10.)(15.8,11.5)(0.,){/Straight}{1}
\FALabel(14.3877,11.4607)[br]{$t$}
\FAProp(18.2,13.5)(15.8,11.5)(-0.8,){/Straight}{-1}
\FALabel(18.3123,10.8293)[tl]{$t$}
\FAProp(18.2,13.5)(15.8,11.5)(0.8,){/Cycles}{0}
\FALabel(15.6877,14.1707)[br]{$g$}
\FAVert(6.,10.){0}
\FAVert(18.2,13.5){0}
\FAVert(14.,10.){0}
\FAVert(15.8,11.5){0}
\end{feynartspicture}



==> DIAGRAMS/loop.tex <==
\unitlength=0.3bp%
%
%
% LOOP UNCUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}
%
%
\hspace{0.5cm}  % LOOP DOUBLE CUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\myblue
\FAProp(13.75,15.)(13.75,5.)(0.,){/ScalarDash}{0}
\black
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}
%
%
\hspace{0.5cm}  % LOOP SINGLE CUT
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(21.,10.)(16.5,10.)(0.,){/Straight}{-1}
\FALabel(21.25,11.07)[b]{\tiny $t \; (K, c)$}
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAProp(16.5,10.)(11.,10.)(-0.8,){/Straight}{-1}
\myblue
\FAProp(13.75,10.5)(13.75,5.)(0.,){/ScalarDash}{0}
\black
\FAProp(16.5,10.)(11.,10.)(0.8,){/Cycles}{0}
\FAVert(6.5,10.){-1}
\FALabel(6.5,10.)[]{\tiny $\mathcal{A}$}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}


==> DIAGRAMS/totDS.tex <==
\unitlength=0.47bp%
%
%
%   LOOP DOUBLE 
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(12.6,10.)(19.,10.)(0.,){/Cycles}{0}
\FAProp(19.,16.)(12.6,10.5)(0.,){/Straight}{1}
\FAProp(12.6,9.5)(19., 4.)(0.,){/Cycles}{0}
\FALabel(17.5,15.8)[b]{\scriptsize $2^-$}
\FALabel(19.,5.97)[b]{\scriptsize $4^-$}
\FALabel(19.,11.07)[b]{\scriptsize $3^-$}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{-1}
\FALabel(1.,11.07)[b]{\scriptsize $1^-$}
\FAProp(12.5,10.)(6.5,10.)(0.8,){/Straight}{1}
\FAProp(12.5,10.)(6.5,10.)(-0.8,){/Cycles}{0}
\FAVert(12.5,10.){-3}
\FAVert(6.5,10.){0}
\FAProp(9.25,15.)(9.25,5.)(0.,){/ScalarDash}{0}
\FALabel(9.3,0.)[b]{$\Delta_{2,k} A^{R}$}
\FAProp(5.7,8.)(8.3,6.5)(0.2,){/Straight}{-1}
\FALabel(7.,5.25)[b]{\scriptsize $\ell$}
\end{feynartspicture}
%
%
\hspace{0.61cm} % TREE LEFT
%
% 
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(12.6,10.)(19.,10.)(0.,){/Cycles}{0}
\FAProp(19.,16.)(12.6,10.5)(0.,){/Straight}{1}
\FAProp(12.6,9.5)(19., 4.)(0.,){/Cycles}{0}
\FALabel(17.5,15.8)[b]{\scriptsize $2^-$}
\FALabel(19.,5.97)[b]{\scriptsize $4^-$}
\FALabel(19.,11.07)[b]{\scriptsize $3^-$}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{-1}
\FALabel(1.,11.07)[b]{\scriptsize $1^-$}
\FAProp(12.5,10.)(6.5,10.)(-0.8,){/Straight}{1}
\FAProp(12.5,10.)(6.5,10.)(0.8,){/Cycles}{0}
\FAProp(5.7,12.)(8.3,13.5)(-0.2,){/Straight}{-1}
\FALabel(7.,14.75)[t]{\scriptsize $\ell$}
\FAVert(12.5,10.){-3}
\FAVert(6.5,10.){0}
\FAProp(9.25,15.)(9.25,5.)(0.,){/ScalarDash}{0}
\FALabel(9.3,0.)[b]{$\Delta_{2,k} A^{L}$}
\end{feynartspicture}
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FALabel(0.,10.)[l]{\scriptsize $\mathcal{A}$}
%\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
%\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
%\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
%\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
%\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
%\FAProp(11.,10.)(16.,14.)(0.,){/Cycles}{0}
%\FALabel(19.3,13.2)[t]{\scriptsize $g (\ell, A)$}
%\FAProp(11.,10.)(16., 6.)(0.,){/Straight}{1}
%\FALabel(20.,6.8)[b]{\scriptsize $t (k-\ell, c')$}
%\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
%\FALabel(9.25,11.07)[b]{\scriptsize $\mathcal P$}
%\FAVert(6.5,10.){-1}
%\FALabel(6.5,10.)[]{\scriptsize $\mathcal{A}$}
%\FAVert(16.5,10.){0}
%\FAVert(11.,10.){0}
%\FALabel(10.,0.)[b]{ $\mathcal{M}_L$}
%\end{feynartspicture}
%
%
%\hspace{0.55cm}  % TREE RIGHT
%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,14.)(7.5,10.)(0.,){/Cycles}{0}
%\FALabel(3.37021,11.6903)[tr]{\scriptsize $g (\ell, A)$}
%\FAProp(0.,6.)(7.5,10.)(0.,){/Straight}{1}
%\FALabel(4.12979,6.69032)[tl]{\scriptsize $t (k-\ell, c')$}
%\FAProp(7.5,10.)(15.,10.)(0.,){/Straight}{1}
%\FALabel(13.25,11.07)[b]{\scriptsize $t (k,c)$}
%\FAVert(7.5,10.){0}
%\FALabel(7.,0.)[b]{ $\mathcal{M}_R$}
%\end{feynartspicture}

==> DIAGRAMS/totTS.tex <==
\unitlength=0.33bp%
%
% 
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(8.,10.)(8.,18.)(0.,){/Straight}{-1}
\FALabel(9.4,18)[]{\scriptsize $2$}
\FAProp(8.,10.)(15.6085,12.4721)(0.,){/Cycles}{0}
\FALabel(15.,13.8)[]{\scriptsize $3$}
\FAProp(8.,10.)(0.3915,12.4721)(0.,){/Cycles}{0}
\FALabel(1.,13.8)[]{\scriptsize $\ell$}
\FAProp(8.,10.)(12.7023,3.52786)(0.,){/Cycles}{0}
\FALabel(14.,3.5)[]{\scriptsize $4$}
\FAProp(8.,10.)(3.2977,3.52786)(0.,){/Straight}{1}
%\FALabel(2.,3.5)[]{\scriptsize D}
\FALabel(0.7,3.5)[]{\scriptsize $\ell +k_1$}
\FAVert(8.,10.){-3}
\FALabel(19.0,10)[]{=}
\end{feynartspicture}
%
%
\hspace{0.5cm}
%
% 
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(8.,10.)(8.,18.)(0.,){/Cycles}{0}
\FALabel(9.4,18)[]{\scriptsize $3$}
\FAProp(8.,10.)(15.6085,12.4721)(0.,){/Cycles}{0}
\FALabel(15.,13.8)[]{\scriptsize $4$}
\FAProp(8.,10.)(0.3915,12.4721)(0.,){/Straight}{-1}
\FALabel(1.,13.8)[]{\scriptsize $2$}
\FAProp(8.,10.)(12.7023,3.52786)(0.,){/Cycles}{0}
\FALabel(14.,3.5)[]{\scriptsize $\ell$}
\FAProp(8.,10.)(3.2977,3.52786)(0.,){/Straight}{1}
%\FALabel(2.,3.5)[]{\scriptsize D}
\FALabel(0.7,3.5)[]{\scriptsize $\ell +k_1$}
\FAVert(8.,10.){-3}
\FALabel(-2.70,10)[]{--}
\end{feynartspicture}
%
%
%
% 
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(8.,10.)(8.,18.)(0.,){/Cycles}{0}
\FALabel(9.4,18)[]{\scriptsize $3$}
\FAProp(8.,10.)(15.6085,12.4721)(0.,){/Cycles}{0}
\FALabel(15.,13.8)[]{\scriptsize $\ell$}
\FAProp(8.,10.)(0.3915,12.4721)(0.,){/Straight}{-1}
\FALabel(1.,13.8)[]{\scriptsize $2$}
\FAProp(8.,10.)(12.7023,3.52786)(0.,){/Cycles}{0}
\FALabel(14.,3.5)[]{\scriptsize $4$}
\FAProp(8.,10.)(3.2977,3.52786)(0.,){/Straight}{1}
%\FALabel(2.,3.5)[]{\scriptsize D}
\FALabel(0.7,3.5)[]{\scriptsize $\ell +k_1$}
\FAVert(8.,10.){-3}
\FALabel(-2.70,10)[]{--}
\end{feynartspicture}
%
%
%
% 
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(8.,10.)(8.,18.)(0.,){/Cycles}{0}
\FALabel(9.4,18)[]{\scriptsize $\ell$}
\FAProp(8.,10.)(15.6085,12.4721)(0.,){/Cycles}{0}
\FALabel(15.,13.8)[]{\scriptsize $3$}
\FAProp(8.,10.)(0.3915,12.4721)(0.,){/Straight}{-1}
\FALabel(1.,13.8)[]{\scriptsize $2$}
\FAProp(8.,10.)(12.7023,3.52786)(0.,){/Cycles}{0}
\FALabel(14.,3.5)[]{\scriptsize $4$}
\FAProp(8.,10.)(3.2977,3.52786)(0.,){/Straight}{1}
%\FALabel(2.,3.5)[]{\scriptsize D}
\FALabel(0.7,3.5)[]{\scriptsize $\ell +k_1$}
\FAVert(8.,10.){-3}
\FALabel(-2.70,10)[]{--}
%\FALabel(19.0,10)[]{=}
\end{feynartspicture}
%
%

==> DIAGRAMS/treeL.tex <==
\unitlength=0.22bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,12.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,10.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,8.)(6.5,10.)(0.,){/Straight}{0}
\FAProp(0.,6.)(6.5,10.)(0.,){/Straight}{0}
%
\FAProp(11.,10.)(16.,14.)(0.,){/Cycles}{0}
\FALabel(19.3,13.2)[t]{\tiny $g (\ell, A)$}
\FAProp(11.,10.)(16., 6.)(0.,){/Straight}{1}
\FALabel(22.,6.8)[b]{\tiny $t (K-\ell, c')$}
%
\FAProp(6.5,10.)(11.,10.)(0.,){/Straight}{1}
\FAVert(6.5,10.){-1}
\FAVert(16.5,10.){0}
\FAVert(11.,10.){0}
\end{feynartspicture}



==> DIAGRAMS/treeR.tex <==
\unitlength=0.22bp%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,14.)(7.5,10.)(0.,){/Cycles}{0}
\FALabel(3.37021,11.6903)[tr]{\tiny $g (\ell, A)$}
\FAProp(0.,6.)(7.5,10.)(0.,){/Straight}{1}
\FALabel(4.12979,6.69032)[tl]{\tiny $t (K-\ell, c')$}
\FAProp(7.5,10.)(15.,10.)(0.,){/Straight}{1}
\FALabel(13.25,11.07)[b]{\tiny $t (K,c)$}
\FAVert(7.5,10.){0}
\end{feynartspicture}



==> DIAGRAMS/ttggCT.tex <==
%\unitlength=0.42bp%
\unitlength=0.42bp
%
%
%
%\scriptsize
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,12.3)[tr]{\scriptsize$2$}
\FAProp(0.,5.)(3.,6.5)(0.,){/Straight}{-1}
\FALabel(2.01229,5.2)[tl]{\scriptsize$1$}
\FAProp(20.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.7)[br]{\scriptsize$3$}
\FAProp(20.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,7.5)[bl]{\scriptsize$4$}
\FAProp(3.,6.5)(10.,10.)(0.,){/Straight}{-1}
%\FALabel(5.01229,8.03926)[tl]{$t$}
%\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,11.77)[b]{$g$}
\FAVert(10.,10.){-3}
%\FAVert(14.,10.){0}
\FAVert(4.,7.0){2}
\FALabel(10.0,0.)[]{$D_a$}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(4.,13.0)(0.,){/Straight}{1}
\FALabel(0.987714,13.0393)[tr]{\scriptsize$2$}
\FAProp(0.,5.)(10.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.2)[tl]{\scriptsize$1$}
\FAProp(20.,15.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.7)[br]{\scriptsize$3$}
\FAProp(20.,5.)(10.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,7.5)[bl]{\scriptsize$4$}
\FAProp(4.,13.0)(10.,10.)(0.,){/Straight}{1}
%\FALabel(5.01229,11.9607)[bl]{$t$}
%\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,8.93)[t]{$g$}
\FAVert(10.,10.){-3}
\FAVert(4.,13.0){2}
\FALabel(10.0,0.)[]{$D_b$}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{\scriptsize$2$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{\scriptsize$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{\scriptsize$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{\scriptsize$4$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{-1}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{1}
%\FALabel(8.93,8.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){2}
\FALabel(10.0,0.)[]{$D_c$}
\end{feynartspicture}



==> DIAGRAMS/ttggCT_copy.tex <==
%\unitlength=0.42bp%
\unitlength=0.25bp
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\scriptsize
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$2$}
\FAProp(0.,5.)(3.,7.5)(0.,){/Straight}{-1}
\FALabel(2.01229,5.53926)[tl]{$1$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$3$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$4$}
\FAProp(3.,7.5)(6.,10.)(0.,){/Straight}{-1}
%\FALabel(5.01229,8.03926)[tl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,11.77)[b]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,7.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$2$}
\FAProp(0.,5.)(5.,5.5)(0.,){/Straight}{-1}
\FALabel(2.65423,4.18769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(5.,5.5)(10.,6.)(0.,){/Straight}{-1}
%\FALabel(7.65423,4.68769)[t]{$t$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
%\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(5.,5.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(3.,12.5)(0.,){/Straight}{1}
\FALabel(0.987714,13.0393)[tr]{$2$}
\FAProp(0.,5.)(6.,10.)(0.,){/Straight}{-1}
\FALabel(3.51229,6.78926)[tl]{$1$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$3$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$4$}
\FAProp(3.,12.5)(6.,10.)(0.,){/Straight}{1}
%\FALabel(5.01229,11.9607)[bl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
%\FALabel(10.,8.93)[t]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,12.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.,14.5)(0.,){/Straight}{1}
\FALabel(2.65423,15.8123)[b]{$2$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(5.,14.5)(10.,14.)(0.,){/Straight}{1}
%\FALabel(7.65423,15.3123)[b]{$t$}
\FAProp(10.,6.)(10.,14.)(0.,){/Straight}{-1}
%\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,6.){0}
\FAVert(10.,14.){0}
\FAVert(5.,14.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$2$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$1$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$3$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$4$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{-1}
%\FALabel(11.07,12.)[l]{$t$}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{1}
%\FALabel(8.93,8.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){2}
\end{feynartspicture}



==> DIAGRAMS/ttggCTdef.tex <==
\unitlength=0.42bp%
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,10.)(9.,10.)(0.,){/ScalarDash}{0}
%\FALabel(2.5,9.18)[t]{\scriptsize $H (k_1)$}
%\FAProp(18.,15.)(9.,10.)(0.,){/Straight}{-1}
%\FALabel(13.2273,13.3749)[br]{\scriptsize $b (k_2, c_2)$}
%\FAProp(18.,5.)(9.,10.)(0.,){/Straight}{1}
%\FALabel(13.2273,6.62506)[tr]{\scriptsize $b(k_3,c_3)$}
%\FAVert(9.,10.){-1}
%\FALabel(9.,10.)[]{\scriptsize $L$}
%\end{feynartspicture}
%
%
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,10.)(0.,){/Straight}{1}
\FALabel(2.48771,11.7893)[tr]{$t$}
\FAProp(0.,5.)(3.,7.5)(0.,){/Straight}{-1}
\FALabel(2.01229,5.53926)[tl]{$t$}
\FAProp(20.,15.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(16.4877,13.2107)[br]{$g$}
\FAProp(20.,5.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(17.5123,8.21074)[bl]{$g$}
\FAProp(3.,7.5)(6.,10.)(0.,){/Straight}{-1}
\FALabel(5.01229,8.03926)[tl]{$t$}
\FAProp(6.,10.)(14.,10.)(0.,){/Cycles}{0}
\FALabel(10.,11.77)[b]{$g$}
\FAVert(6.,10.){0}
\FAVert(14.,10.){0}
\FAVert(3.,7.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$t$}
\FAProp(0.,5.)(5.,5.5)(0.,){/Straight}{-1}
\FALabel(2.65423,4.18769)[t]{$t$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$g$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$g$}
\FAProp(5.,5.5)(10.,6.)(0.,){/Straight}{-1}
\FALabel(7.65423,4.68769)[t]{$t$}
\FAProp(10.,14.)(10.,6.)(0.,){/Straight}{1}
\FALabel(8.93,10.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(5.,5.5){2}
\end{feynartspicture}
%
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(10.,14.)(0.,){/Straight}{1}
\FALabel(4.84577,13.4377)[t]{$t$}
\FAProp(0.,5.)(10.,6.)(0.,){/Straight}{-1}
\FALabel(5.15423,4.43769)[t]{$t$}
\FAProp(20.,15.)(10.,14.)(0.,){/Cycles}{0}
\FALabel(14.8458,15.5623)[b]{$g$}
\FAProp(20.,5.)(10.,6.)(0.,){/Cycles}{0}
\FALabel(15.1542,6.56231)[b]{$g$}
\FAProp(10.,10.)(10.,14.)(0.,){/Straight}{-1}
\FALabel(11.07,12.)[l]{$t$}
\FAProp(10.,10.)(10.,6.)(0.,){/Straight}{1}
\FALabel(8.93,8.)[r]{$t$}
\FAVert(10.,14.){0}
\FAVert(10.,6.){0}
\FAVert(10.,10.){2}
\end{feynartspicture}


